Equivalence Checking of Quantum Circuits by Model Counting

Verifying equivalence between two quantum circuits is a hard problem, that is nonetheless crucial in compiling and optimizing quantum algorithms for real-world devices. This paper gives a Turing reduction of the (universal) quantum circuits equivalence problem to weighted model counting (WMC). Our starting point is a folklore theorem showing that equivalence checking of quantum circuits can be done in the so-called Pauli-basis. We combine this insight with a WMC encoding of quantum circuit simulation, which we extend with support for the Toffoli gate. Finally, we prove that the weights computed by the model counter indeed realize the reduction. With an open-source implementation, we demonstrate that this novel approach can outperform a state-of-the-art equivalence-checking tool based on ZX calculus and decision diagrams.

==> preamble.tex <==

\RequirePackage{color}


\RequirePackage{physics}
\RequirePackage{graphicx}
\RequirePackage{amsmath}

\RequirePackage{algorithm}
\RequirePackage[noend]{algpseudocode}

\RequirePackage{amssymb}
\RequirePackage{braket}

\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{thmtools}
\RequirePackage{xspace}
\RequirePackage{multirow}
\usepackage{colortbl}
\RequirePackage{stmaryrd}
\RequirePackage[colorlinks,citecolor=blue!60!black!70,linkcolor=blue!60!black!70]{hyperref}%
\usepackage{appendix}
\RequirePackage{hyperref}
\RequirePackage{subcaption}
\RequirePackage{mathrsfs}
\RequirePackage[english]{babel}
\RequirePackage{pgfplots}
\RequirePackage{calc}
\RequirePackage{nicefrac}
\RequirePackage{todonotes}
\RequirePackage{complexity}
\RequirePackage{tikz}
\usetikzlibrary{shapes,backgrounds,calc,arrows,automata}
\usetikzlibrary{graphs,quotes}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{shapes,backgrounds,calc,arrows}
\RequirePackage{soul}
\RequirePackage{wrapfig}
\let\clipbox\relax
\pgfplotsset{compat=1.18}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{empheq}
\usepackage{amssymb}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
\usepackage{hyperref}
\usepackage{tabularx}
\usepackage{etoolbox}
\usepackage{arydshln}
\usepackage{mathtools}



\newcommand{\algstrut}[1][\algruledefaultfactor]{\vrule width 0pt
depth .25\baselineskip height #1\baselineskip\relax}


\newcommand*{\algrule}[1][\algorithmicindent]{\hspace*{.5em}\vrule\vrule
width 0pt height .75\baselineskip depth .25\baselineskip\hspace*{\dimexpr#1-.5em}}

\makeatletter
\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0%
    \ifx\ALG@text\ALG@x@notext%
    \addvspace{-3pt}%
    \else
    \unskip
    \ALG@printindent@tempcnta=1
    \loop
    \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
    \advance \ALG@printindent@tempcnta 1
    \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax%
    \repeat
    \fi
    \fi
}
\usepackage{etoolbox}
\usepackage{pifont}
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother

\AtBeginEnvironment{algorithmic}{\lineskip-2pt}


\newcommand*\Stateh{\State \algstrut[1]}


\interfootnotelinepenalty=10000

\RequirePackage[bottom,symbol]{footmisc} 
\RequirePackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$ {\footnotesize #1}}

\setlength{\parskip}{7pt}
\setlength{\parindent}{0pt}

\newcommand{\innerprod}[2]{\langle #1 | #2 \rangle}

\newcommand{\unit}{I}
\def\X{X}
\def\Y{Y}
\def\Z{Z}
\newenvironment{algo}[1][Algorithm]
    {\begin{center} 
    \begin{tabular}{|p{0.9\textwidth}|} 
    \hline 
    \vspace{0.1\baselineskip} 
    \textbf{#1}\\} 
    { 
    \\\hline 
    \end{tabular} 
    \end{center} 
    \vspace{\baselineskip} 
    } 


\newcommand{\diagonal}[1]{\begin{smallmat}1 & 0 \\ 0 & #1\end{smallmat}}
\newcommand{\antidiagonal}[1]{\begin{smallmat}0 & #1 \\ 1 & 0\end{smallmat}}

\makeatletter
\renewcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%
\makeatother

\usepackage{caption}
\usepackage{MnSymbol}
\usepackage[makeroom]{cancel}
\usepackage{quantikz}

\renewcommand\sectionautorefname{Section}
\renewcommand\subsectionautorefname{Section}
\renewcommand\subsubsectionautorefname{Section}
\renewcommand\figureautorefname{Figure}
\renewcommand\tableautorefname{Table}
\newcommand\exampleautorefname{Example}
\newcommand\algorithmautorefname{Algorithm}
\renewcommand\appendixautorefname{Appendix}
\newcommand*{\Appendixautorefname}{Appendix}
\renewcommand\itemautorefname{Item}
\renewcommand\theoremautorefname{Theorem}
\renewcommand\equationautorefname{Eq.}

